LiteQSign: Lightweight and Quantum-Safe Signatures for Heterogeneous IoT Applications

The rapid proliferation of resource-constrained IoT devices across sectors like healthcare, industrial automation, and finance introduces major security challenges. Traditional digital signatures, though foundational for authentication, are often infeasible for low-end devices with limited computational, memory, and energy resources. Also, the rise of quantum computing necessitates post-quantum (PQ) secure alternatives. However, NIST-standardized PQ signatures impose substantial overhead, limiting their practicality in energy-sensitive applications such as wearables, where signer-side efficiency is critical. To address these challenges, we present LightQSign (LightQS), a novel lightweight PQ signature that achieves near-optimal signature generation efficiency with only a small, constant number of hash operations per signing. Its core innovation enables verifiers to obtain one-time hash-based public keys without interacting with signers or third parties through secure computation. We formally prove the security of LightQSign in the random oracle model and evaluate its performance on commodity hardware and a resource-constrained 8-bit AtMega128A1 microcontroller. Experimental results show that LightQSign outperforms NIST PQC standards with lower computational overhead, minimal memory usage, and compact signatures. On an 8-bit microcontroller, it achieves up to 1.5-24x higher energy efficiency and 1.7-22x shorter signatures than PQ counterparts, and 56-76x better energy efficiency than conventional standards-enabling longer device lifespans and scalable, quantum-resilient authentication.

==> Chapters/trash.tex <==
%\vspace{2pt}
%{\em There is a significant need for lightweight post-quantum signatures that respect the strict memory, computation, and bandwidth limitations of resource-constrained IoT applications}. In particular, the heavy overhead of current post-quantum signatures on embedded devices is a severely limiting factor in their real-life deployment. In this work,  we  aim to answer the following research questions:
%
%\textit{(i) Is it possible to achieve efficient quantum-safe signing with only symmetric cryptographic operations?} \textit{(ii) Is it possible to permit efficient signing without imposing non-conventional and risky assumptions on the verifier like non-colluding multiple servers or third parties storing secret keys, suffering from key escrow?} \textit{(iii) Can we meet these requirements in a multi-user setting to scale IoTs?}


%\underline{$\bullet$ \em All above properties without introducing additional assum-} \underline{\em -ptions on verifier}: Several previous techniques attempt to achieve the above desirable properties by introducing new security and/or model assumptions on the verifier. For example, 

%\vspace{8pt}
%Standard digital signatures (e.g., RSA \cite{rivest1978method}, ECDSA \cite{johnson2001elliptic}) depend on traditional cryptographic assumptions, such as Elliptic Curve Discrete Logarithm Problem (ECDLP). However, these standard digital signatures involve computationally intensive operations, such as modular exponentation or EC scalar multiplication. These latter do not suit the stringent resource constraints of IoT devices in terms of processing and memory workloads. 

%The emergence of quantum computers significantly increases the challenges associated with implementing digital signatures in resource-limited IoT devices. Traditional cryptographic methods, such as those based on number theoretic assumptions (e.g., ECDLP), are vulnerable to quantum attacks using Shor’s algorithm \cite{shor1999polynomial}. This vulnerability has drawn considerable attention from industry, academia, and government sectors \cite{darzi2023envisioning}. Notably, the NIST’s Post-Quantum Cryptography (PQC) standardization process selected specific digital signatures—CRYSTALS-Dilithium as the Module-Lattice-Based Digital Signature Standard (FIPS 204) and SPHINCS+ as the Stateless Hash-Based Digital Signature Standard (FIPS 205) \cite{nist-pqc}. However, despite their robustness, these post-quantum digital signatures are not optimized for resource-limited IoT systems. They require significantly more computational power and produce larger signature sizes than conventional digital signatures. Experimental data (refer to Table \ref{tab:embeddedperformance}, Section \ref{sec:performance}) indicate that these signatures impose substantial computational demands, making them impractical for resource-limited IoT devices that need to operate efficiently under constraints of battery life, processing power, and bandwidth \cite{li2019privacy}.
